The DUNE Far Detector Interim Design Report, Volume 3: Dual-Phase Module

The DUNE IDR describes the proposed physics program and technical designs of the DUNE far detector modules in preparation for the full TDR to be published in 2019. It is intended as an intermediate milestone on the path to a full TDR, justifying the technical choices that flow down from the high-level physics goals through requirements at all levels of the Project. These design choices will enable the DUNE experiment to make the ground-breaking discoveries that will help to answer fundamental physics questions. Volume 3 describes the dual-phase module's subsystems, the technical coordination required for its design, construction, installation, and integration, and its organizational structure.

==> common/intro.tex <==
% Intro shared by all subsections NOT USED IN TECNICAL PROPOSAL

\section{An International Physics Program}

The global neutrino physics community is developing a multi-decade
physics program to measure unknown parameters of the Standard Model of
particle physics and search for new phenomena.  The program will be carried out as an international,
leading-edge, dual-site experiment for neutrino science and proton decay studies, which 
is known as the Deep Underground Neutrino Experiment (DUNE).
The detectors for this experiment will be designed, built, commissioned and operated by the international DUNE Collaboration. The facility required to support this experiment, the Long-Baseline Neutrino Facility (LBNF), is hosted by Fermilab and its design and construction is organized as a DOE/Fermilab project incorporating international partners. Together LBNF and DUNE will comprise the world's highest-intensity neutrino beam at Fermilab, in Batavia, IL, a high-precision near detector on the Fermilab site, a massive liquid argon time-projection chamber (LArTPC) far detector installed deep underground at the Sanford Underground Research Facility (SURF) \SI{1300}{\km} away in Lead, SD, and all of the conventional and technical facilities necessary to support the beamline and detector systems. 


The strategy for executing the experimental program presented in this Technical
Design Report (TDR) has been developed to meet the requirements 
set out in the P5 report~\cite{p5report} and takes into account the recommendations of the European Strategy for Particle Physics~\cite{ESPP-2012}. It adopts a model where U.S. and international funding agencies 
share costs on the DUNE detectors, and CERN and other participants provide in-kind contributions 
to the supporting infrastructure of LBNF. LBNF and DUNE have been and will remain tightly coordinated as DUNE collaborators 
develop the detectors and infrastructure that will carry out the scientific program.
  
The scope of LBNF is
\begin{itemize}
\item an intense neutrino beam aimed at the far site,
\item a beamline measurement system
\item conventional facilities at both the near and far sites, and
\item cryogenics infrastructure to support the DUNE detector at the far site.
\end{itemize}

The DUNE detectors include
\begin{itemize}
\item a high-performance neutrino detector 
located a few hundred meters downstream of the neutrino source, and
\item a massive liquid argon time-projection chamber (LArTPC) neutrino detector located deep underground at the far site.
\end{itemize}

With the facilities provided by LBNF and the detectors provided by
DUNE, the DUNE Collaboration proposes to mount a focused attack on the
puzzle of neutrinos with broad sensitivity to neutrino oscillation
parameters in a single experiment.  The focus of the scientific
program is the determination of the neutrino mass hierarchy and the
explicit demonstration of leptonic CP violation, if it exists, by
precisely measuring differences between the oscillations of muon-type
neutrinos and antineutrinos into electron-type neutrinos and
antineutrinos, respectively. Siting the far detector deep underground
will provide exciting additional research opportunities in nucleon
decay, studies utilizing atmospheric neutrinos, and neutrino
astrophysics, including measurements of neutrinos from a core-collapse
supernova should such an event occur in our galaxy during the
experiment's lifetime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The LBNF/DUNE Technical Design Report Volumes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Roadmap of the TDR}

The LBNF/DUNE TDR describes the proposed physics program and \fixme{baselined?}
technical designs.

The TDR is composed of \fixme{some number of} volumes and is supplemented by several annexes that 
provide details on the physics program and technical designs. The volumes are as follows

\begin{itemize}
\item \volintro{}\cite{tdr-vol-1} provides an executive summary of and strategy for the experimental 
program and introduces the TDR.
\item \volphys{}\cite{tdr-vol-2} outlines the scientific objectives and describes the physics studies that 
the DUNE Collaboration will undertake to address them.
\item \vollbnf{}\cite{tdr-vol-3} describes the LBNF Project, which includes design and construction of the 
beamline at Fermilab, the conventional facilities at both Fermilab and SURF, and the cryostat
 and cryogenics infrastructure required for the DUNE far detector.
\item \voldunenear{}\cite{tdr-vol-4}  describes design, construction and 
commissioning of the DUNE near detector. 
\item \voldunefar{}\cite{tdr-vol-5}  describes design, construction and 
commissioning of the DUNE far detectors.
\end{itemize}

More detailed information for each of these volumes is provided in a set of annexes listed on LBNF and DUNE's shared  \href{https://web.fnal.gov/project/LBNF/SitePages/Proposals%20and%20Design%20Reports.aspx}{\textit{Proposals and Design Reports} page}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{About this Volume}  <----- follows in overview chapter file of indiv volume



==> far-detector-dual-phase/chapter-fddp-performance.tex <==
\chapter{Detector Performance}
\label{ch:fddp-perform}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{??}
\label{sec:fddp-perform-??}



==> far-detector-generic/chapter-fd-coordination/dss.tex <==
\subsection{Detector Support System}

The \dword{dss} provides the structural support for the \dword{spmod}
inside the cryostat.  It also provides the necessary
infrastructure to move the detector elements into location during
assembly. As the \dword{dss} is a new design and is quite different
from the \dword{pdsp} \dword{dss} it is described in some detail in this
section. The detector elements supported by the \dword{dss} include
the \dwords{ewfc}, the \dwords{apa}, and the \dwords{cpa} with
top and bottom \dword{fc} panels.  The \dword{dss} is supported by the
cryostat outer steel structure through a series of \fdth{}s that
cross through the cryostat insulation and are anchored with flanges on
the cryostat roof. Inside the cryostat a series of stainless steel
I-beams are connected to the \fdth{}s and used to support the
detector. The \dword{dss} defines the location of the detector inside
the cryostat and it also defines how the detector elements
move and contract as the detector is brought to \dword{lar}
temperature. The design of the \dword{dss} encompasses the overall
structural design of the \dword{detmodule} as only after the elements are
mounted to the \dword{dss} and are connected together do they make a
unified mechanical structure. The requirements of the \dword{dss} are
as follows:
\begin{itemize}
 \setlength\itemsep{1mm}
\setlength{\parsep}{1mm}
\setlength{\itemsep}{-5mm}
% \small
\item Support the weight of the detector.
\item Accommodate cryostat roof movement during filling, testing, and operation.
\item Accommodate variation in \fdth locations and
  variation in the flange angles due to installation tolerances and
  loading on the warm structure.
\item Accommodate shrinkage of the detector and \dword{dss} from ambient
  temperature to \dword{lar} temperature.
\item Define the position of the detector components relative to each other. 
\item Provide electrical connection to the cryostat ground and remain electrically isolated from the detector.
\item Allow for the support penetrations to be purged with gaseous argon to prevent contaminants from diffusing back into the liquid. 
\item Ensure that the instrumentation cabling does not interfere with the \dword{dss}.
\item Consist entirely of components that can %Components must 
be installed through the \dword{tco}.
\item %Design to m
Meet AISC-360 or appropriate codes required at \surf.
\item %Design to m
Meet seismic requirements one mile underground at \surf.
\item Consist entirely of %All materials must be 
materials that are compatible for operation in ultrapure \dword{lar}.
\item Ensure that beams are completely submerged in \dword{lar}.
\item Ensure that detector components are not less than \SI{400}{mm} from the membrane flat surface.
\item Ensure that the supports do not interfere with the cryostat I-beam structures.
\item Ensure %Design such 
that the detector's lower \dword{gp} is above the cryogenic piping and the top of the \dword{dss} beams are submerged in \dword{lar} while leaving a \SI{4}{\%} ullage at the top of the cryostat.
\item Include the infrastructure necessary to move the \dword{apa} and
  \dword{cpa}-\dword{fc} assemblies from outside the cryostat through the
  \dword{tco} and to the correct position.
\end{itemize}

Figure~\ref{fig:DSS} (left) shows the \dword{dss} structure; there are
five rows of supports for the alternating rows of
\dword{apa}-\dword{cpa}-\dword{apa}-\dword{cpa}-\dword{apa}.  The
\dword{dss} is connected to the warm structure at a flange that is
mounted on the outside of the cryostat.  Figure~\ref{fig:DSS} (right)
shows the layout of these structural \fdth{}s.  The \dword{dss}
consists of pairs of \fdth{}s that support \SI{6.4}{m}-long
S8x18.4 stainless steel I-beam sections. The proposed design of the
\dword{dss} has \num{10} I-beam segments per row for a total of
\num{50} I-beam segments. Each I-beam is suspended on both ends by
rods from \fdth{}s that penetrate the roof.  %In the cold condition
When cold, each beam shrinks, causing gaps to form between
\dwords{apa} that are adjacent but supported on separate beams.
\dwords{apa} that are supported on the same beam will not have gaps
develop because both the beam and \dwords{apa} are stainless steel so
they shrink together.  Each beam is supported by a nearly
\SI{2}{m} long rod that allows the beam support to move as the beam
contracts.
%\fixme{too much detail}
%The feedthrough consists of a flange and $8 ^{''}$ OD structural tube
%welded to it that extends through the cryostat insulation.  There is a
%nominal \SI{10}{mm} gap between the OD of the tube and the ID of the
%clearance tube in the cryostat.  The purpose of the $8 ^{''}$ tube is
%to provide lateral support to the I-beams during installation.
%Running down the center of the feedthrough is a $1^{"}$ diameter rod that
%is supported at a swivel washer at the flange and then supports the
%I-beam at a clevis.  The gas seal is obtained by Conflat Flange and a
%bellows that seals around the swivel washer.  The lateral position of
%the rod can be adjusted to adjust the height of the \dword{dss} I-beams.

\begin{dunefigure}[\threed model of the \dword{dss} ]{fig:DSS}
  {\threed model of the \dword{dss} showing the entire
  structure on the left along with one row of \dword{apa} and
  \dword{cpa}-\dword{fc} at each end. The right panel is a zoomed image
  showing the connections between the vertical supports and the
  horizontal I-beams.}
\includegraphics[width=.49\textwidth]{DSS-1.pdf}
 \includegraphics[width=.49\textwidth]{DSS-2.pdf}
\end{dunefigure}

%\begin{figure}[htbp]
%\begin{center}
%\begin{minipage}[c]{0.49\textwidth}
%\includegraphics[width=\textwidth]{far-detector-single-phase/figures/DSS-1.pdf}
%\end{minipage}
%\begin{minipage}[c]{0.49\textwidth}%
%\includegraphics[width=\textwidth]{far-detector-single-phase/figures/DSS-2.pdf}
%\end{minipage}
%end{center}
%\end{figure}


Detector components are installed using a shuttle beam system
illustrated in Figure~\ref{fig:shuttle}.  The last two columns of
\fdth{}s (eastern-most) support temporary beams that run
north-south, perpendicular to the main \dword{dss} beams.  A shuttle
beam
%shown in orange
has trolleys mounted to it and transverses 
north-south until aligned with the required row of \dword{dss} beam.  The last
\dword{apa} or \dword{cpa} in a row is supported by the shuttle beam which is bolted
directly to the \fdth{}s once it is in place.  As the last \dword{cpa} or
\dword{apa} in each row is installed, the north-south beams are removed.

A mechanical interlock system  prevents trolleys
from passing the end of the shuttle beam unless it is aligned with a
corresponding \dword{dss} beam.  The shuttle beam and each detector component are
moved using a motorized trolley.  A commercially available motorized
trolley will be modified as needed to meet the needs of the
installation.

\begin{dunefigure}[\threed models of the shuttle beam end of the \dword{dss}]{fig:shuttle}
  {\threed models of the shuttle beam end of the \dword{dss}. The figures show how an \dword{apa}
is translated into position using the north-south beams until it lines up with the correct
row of I-beams}
\includegraphics[width=.49\textwidth]{/Shuttle-1.pdf}
 \includegraphics[width=.42\textwidth]{shuttle-2.pdf}
\end{dunefigure}


The \dword{dss} installation begins with the placement and alignment of all
the \fdth{}s onto the flanges that are mounted to the warm vessel.
There are \num{25} \fdth{}s per row and five rows for a total of \num{125}
\fdth{}s.  A fixture with a tooling ball is attached to the
clevis of each \fdth.  The $xy$ position in the horizontal plane
and the vertical $z$ position of this tooling ball is defined, then a %.  A
survey is performed to determine the location of each tooling
ball center and $xy$ and $z$ adjustments are made to get the tooling
ball centers to within $\pm$\SI{3}{mm}.  The \SI{6.4}{m} long I-beams are then 
raised and pinned to the clevis.  Each beam weighs roughly \SI{160}{kg} (\SI{350}{lbs}).
A lifting tripod is placed over each of the \fdth{}s
supporting a beam, and a \SI{0.64}{cm} \SI{0.25}{in}  %$1/4 ^{''}$ 
cable is fed through the top
flange of the \fdth down the \SI{14}{m} to the cryostat floor where it
is attached to the I-beam.  The winches on each tripod raise
the beam in unison in order to get it to the correct height to be
pinned to the \fdth clevis.  Once the beams are mounted, a final
survey of the beams takes place to ensure they are properly located and aligned
to each other.

A mock-up of the shuttle system is constructed to test the
mechanical interlock and drive systems for the shuttle beam
for each \dword{detmodule}.  Tests are conducted to evaluate the level of
misalignment between beams that can be tolerated and the amount of
positional control that can be achieved with the motorized trolley. It
is expected this will be finished prior to the \dword{tdr}. At the time of the
\dword{tdr} a larger prototype installation at Ash River will be under
construction. This prototype will use full scale elements and will be
used to develop the installation procedures and to test the
\dword{detmodule} installation process.


==> far-detector-generic/chapter-fd-coordination/outline-sp.tex <==
\chapter{Technical Coordination}
\label{ch:fdsp-coord}

\input{far-detector-generic/chapter-fd-coordination/intro}
\input{far-detector-generic/chapter-fd-coordination/support}
\input{far-detector-generic/chapter-fd-coordination/integration}
\input{far-detector-generic/chapter-fd-coordination/infrastructure}
\input{far-detector-generic/chapter-fd-coordination/dss}
\input{far-detector-generic/chapter-fd-coordination/itf}
\input{far-detector-generic/chapter-fd-coordination/installation}



==> far-detector-generic/chapter-generic-slow-and-cryo/cryo-instrum-cfd.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cryogenics Instrumentation}
\label{sec:fdsp-cryo-instr} % label used for \ref's from single phase sections.
\label{sec:fddp-cryo-instr} % label used for \ref's from dual phase sections.
\label{sec:fdgen-cryo-instr} % label used for \ref's from generic sections.
% Jim G %Carmen

Instrumentation inside the cryostat must ensure that the condition of the \dword{lar} is adequate for operation of the \dshort{tpc}.
This instrumentation includes devices to monitor the impurity level of the argon, e.g., the purity monitors, which provide high precision electron lifetime measurements,
and gas analyzers to ensure that the levels of atmospheric contamination drop below certain limits during the cryostat purging, cooling and filling.
The cryogenics system operation is monitored by temperature sensors deployed in vertical arrays and at the top and bottom of the detector, providing a 
detailed \threed temperature map which can help to predict the \dword{lar} purity across the entire cryostat. The cryogenics instrumentation also includes \lar level monitors and
a system of internal cameras to help in locating sparks in the cryostat and for overall monitoring of the cryostat interior. 
As mentioned in the Introduction, cryogenics instrumentation requires simulation work to identify the proper location for these devices inside the cryostat and
for the coherent analysis of the instrumentation data. 

Figure~\ref{fig:sp-slow-cryo-ports} shows the current map of cryostat ports for the \dword{spmod}, highlighting the ones assigned to instrumentation devices,
as well as the preliminary location for some of these devices. Vertical temperature profilers are located behind the \dwords{apa} ($T_S$) and behind the east end wall ($T_D$).
They are complemented by a coarser \twod grid of sensors at the top and bottom of the cryostat (not shown in the figure). Purity monitors as well as level meters are planned
in each detector side, behind the two front end walls. Inspection cameras will use some of the multipurpose instrumentation ports, but their exact locations are yet to be decided. 

For \dual, additional care must be taken to monitor the gas phase above the liquid level as the temperature and pressure of argon gas affect gas pressure, and consequently the \dword{lem} calibration.  The gas pressure must be monitored to \SI{1}{mbar} precision and accuracy. In proximity to the liquid surface the temperature gradient of the  gas has to be measured with an array of temperature probes with a vertical pitch of about \SI{1}{cm}, and with a coarser \SI{5}{cm} pitch up to the cryostat roof. Each \dword{crp} is also equipped with \num{36} thermometers to sample the temperature across its structure.


\begin{dunefigure}[Cryostat ports]{fig:sp-slow-cryo-ports}
{Cryostat ports and preliminary location of some instrumentation devices. }
\includegraphics[width=0.95\textwidth]{cisc_cryostat_ports.png}
\end{dunefigure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fluid Dynamics Simulations}
\label{sec:fdgen-slow-cryo-cfd}
% P. Strons
% S. Gollapinni

Proper placement of purity monitors, thermometers, and liquid level monitors within the \dword{detmodule} requires knowledge of how \dword{lar} behaves within the cryostat in terms of its fluid dynamics, heat and mass transfer, and distribution of impurity concentrations. 
Fluid motion within the cryostat is driven primarily by small changes in density from thermal gradients, although pump flow rates and inlet and outlet locations also contribute. 
Heat sources include exterior heat from the surroundings, interior heat from the electronics, and heat flow through the pump inlet.

The fluid flow behavior can be determined through simulation of \dword{lar} flow within the detector using ANSYS CFX\footnote{ANSYS\texttrademark{}, \url{https://www.ansys.com/products/fluids/ansys-cfx}.}, a commercially available \dfirst{cfd} code. Such a model must include proper definition of the fluid characteristics, solid bodies and fluid-solid interfaces, and a means for measuring contamination, while still maintaining reasonable solve times.
\fixme{compute times?}
Although simulation of the \dword{detmodule} presents challenges, there exist acceptable simplifications for accurately representing the fluid, the interfacing solid bodies, and variations of contaminant concentrations. Because of the magnitude of thermal variation within the cryostat, modeling of the \dword{lar} is simplified through use of constant thermophysical properties, calculation of buoyant force through use of the Boussinesq Model (using constant a density for the fluid with application of a temperature dependent buoyant force), and a standard shear stress transport turbulence model. Solid bodies that contact the \dword{lar} include the cryostat wall, the cathode planes, the anode planes, the ground plane, and the \dword{fc}. As in previous \dshort{cfd} models of the DUNE \dword{35t} and \dword{protodune} by South Dakota State University (SDSU)\cite{docdb-5915}, the \dword{fc} planes, anode planes, and \dword{gp} can be represented by porous bodies. Since impurity concentration and electron lifetime do not impact the fluid flow, these variables can be simulated as  passive scalars, as is commonly done for smoke releases~\cite{cfd-1} in air or dyes released in liquids.

\fixme{some of this sounds very SP to me -anne}

Significant discrepancies between real data and simulations can have potential impacts on detector performance, as simulation results contribute to decisions about where to locate sensors and monitors, as well as definitions of various calibration quantities. However, methods of mitigating such risks include well established convergence criteria, sensitivity studies, and comparison to results of previous \dshort{cfd} simulation work by SDSU and \fnal. Additionally, the simulation will be improved with input from temperature measurements and validation tests. 

%%%%% Must find better pictures. Just use this for now %%% anne to here Fri 4/27
\begin{dunefigure}[\dshort{cfd} example]{fig:cfd-example}
  {Distribution of temperature on a plane intersecting an inlet (right) and halfway between an inlet and an outlet (left), as predicted by SDSU \dshort{cfd} simulations \cite{docdb-5915}. (See Figure\ \ref{fig:cfd-example-geometry} for geometry.)}
  \includegraphics[height=0.4\textwidth]{cisc_cfd_outlet_z0.png}
  \includegraphics[height=0.4\textwidth]{cisc_cfd_inlet_z52.png}
\end{dunefigure}

Figure~\ref{fig:cfd-example} shows an example of the temperature
distribution on a plane intersecting a \dword{lar} inlet and at a
plane halfway between an inlet and an outlet; the geometry used for
this simulation is shown in Figure~\ref{fig:cfd-example-geometry}.
Note the plume of higher temperature \dword{lar} between the walls and
the outer \dword{apa} on the inlet plane.  The current locations of instrumentation in
the cryostat as shown in Figure~\ref{fig:sp-slow-cryo-ports} were
determined using the temperature and impurity distributions from these
previous simulations.

\begin{dunefigure}[\dshort{cfd} example geometry]{fig:cfd-example-geometry}
  {Layout of the \dshort{tpc} within the cryostat (top) and positions of
    \dword{lar} inlets and outlets (bottom) as modeled in the SDSU
    \dshort{cfd} simulations \cite{docdb-5915}.
    The Y axis is vertical and the X axis is parallel to the \dword{tpc}
    drift direction.
    Inlets are shown in green and outlets are shown in red.}
  \includegraphics[width=0.8\textwidth]{cisc_cfd_cryostat-layout}
  \includegraphics[width=0.8\textwidth]{cisc_cfd_inlet-outlet-layout}
\end{dunefigure}

The initial strategy for the future \dword{cfd} simulation effort is to understand the performance of \dword{protodune} cryogenics system and model the \dwords{fd} to derive requirements for instrumentation devices.
The following is a prioritized set of studies planned to help drive the requirements for other systems:
\begin{enumerate}
\item Review the DUNE \dword{fd} cryogenics system design and verify the current implementation in simulation; this is important to ensure that the model represents what will be built.
\item Model the \dword{pddp}  liquid and gas regions with the same precision as the \dword{fd}. Presently only the liquid model exists. The liquid model is needed to interpret the thermometer data, and the gas model is needed to understand how to place thermometers in the ullage and verify the design of the gaseous argon purge system.
\item Perform a \dword{cfd} study to determine the feasibility of a wier for \dual; this helps to determine if it can be used to clean the \lar surface before the extraction grid is submerged in the \dword{dpmod}.
\item Verify the \dword{spmod} \single \dword{cfd} model in simulation performed by LBNF; this defines the requirements for instrumentation devices (e.g., thermometry).
\item Model the \dword{pddp} liquid and gas regions with the same precision as the \dword{fd}. \fixme{same as a previous bullet}
\end{enumerate}

